First Study of Exclusive Production of Multi-Hadron Final States in Ultraperipheral Collisions

The study of exclusive photoproduction of multi-hadron final states in ultra-peripheral collisions (UPCs) provides a unique avenue to explore quantum chromodynamics (QCD) and the nature of resonances emerging from gluonic interactions. The ALICE Collaboration has recently performed measurements of exclusive four-pion photoproduction using Run 2 data, favoring the presence of two resonances. However, the underlying nature of these resonances remains poorly understood. The enhanced capabilities of the ALICE detector during Run 3 open new opportunities for the study of multi-pion final states, including four and six-pion systems, and processes involving charmonium decays into four-hadron final states. These studies provide an invaluable way to probe the dynamics of highly dense gluonic matter and the interplay between resonant and non-resonant contributions in hadronic systems. In this paper, we outline the ALICE program focused on these analyses.

==> Images/comments.tex <==
new
Submitted by amatyja on Wed, 10/08/2025 - 19:30

Dear Amrit, Thank you for…
Comment
Dear Amrit,

Thank you for your proceedings. Consider some comments from my side which are below, please.

Best regards

Adam
---------------------------------------------------------------------------------







have been extensively studied: add references


This upgrade enabled us to have a continuous readout -> The upgrade enabled a continuous readout

resulted in the observation of new quarkonia decay mode -> What do you have in mind? Add references.

Here we will discuss some recent result -> In this paper, recent results on … will be discussed. (Be more specific)

page 2:

center-of-mass energy of 5.02 TeV -> center-of-mass energy of sqrt{S_{\rm{NN}}}=5.02 TeV

 and no to low activity ->  and almost no activity

The trigger for UPC events required -> The trigger in Run 2 for UPC events required

 During coulomb excitation ->  During Coulomb excitation (you may put a reference here)

multiple photon -> multiple photons

sometime -> sometimes

 wes -> was

You should mention somwhere that ITS and TPC was used to reconstruct tracks 

page 3:

Figure 3 caption:  XnXNn ->  XnXn

Figure 3 caption: give a reference to the original paper 

I would remove "by H.Xing et al. 5 and by W.Zha et al.6" and left just references 5 and 6.

of 200 and 193 GeV. -> of 200 and 193 GeV, respectively.

Figure 4 caption: give a reference to the original paper 

section 3: why there are two references to PDG? Shouldn't be just one and the most recent one?

page 4: 

recent preliminary results from H1 -> give a reference here

MeV/itc2 -> MeV/c2

reference 8 and 13 are the same -> remove 13.

 instead of the pion channel for rho0 events with four pions ->  instead of the two pion final state four pions

Figure 5 caption: give a reference to the original paper 

approx -> \approx

hypothesis compared -> hypothesis is compared

theoretical model KGTT by Klusek-Gawenda and Tapia Takaki 10 -> theoretical model KGTT 10

The comparison result is presented in -> The comparison of KGTT model and the ALICE result is presented in

we can conclude -> one can conclude

From this comparison, -> From the comparison,

Figure 5 caption: give a reference to the original paper

section 4:

 of long shutdown  ->  of the Long Shutdown 

what do you mean "for this period"?

 This opened ->  It opened

possible during Run 2 ->possible in Run 2

page 5:

 can now to carried out -> now, can be carried out

"Additionally, we have observed several new processes in Run 3 for the first time. At UPC 2025,

we presented several performance plots from ultra-peripheral Pb-Pb collisions collected in 2023 at an

center-of-mass energy of 5.36 TeV" -> Additionally, we have observed several new processes in the ultra-peripheral Pb-Pb collisions at the center-of-mass energy of sqrt{s_NN}=5.36 TeV in Run 3 with only 2023 dataset. 

"The Figure 7a shows the invariant mass distribution of the exclusively photoproduced ρ’ in UPCs" -> The invariant mass distribution of the exclusively photoproduced ρ’ in 4 pion channel in UPCs is shown in Fig. 7a.

I do not understand this sentence. Be more specific: The impact of having larger data sample sizes in Run 3 is also illustrated in Fig. section 3.

mesosn -> mesons

Figure  7a caption: 

 - invariant mass of four-pions events -> invariant mass of four-pion events

 - Pb-b -> Pb-Pb

 - ψ_2S ->ψ(2S)

Figure 7 caption:  

 - S_N N -> S_{NN}

 - Could you unify captions of Fig. 7 in sucha way that captions of a) and b) go to the overall caption of Figure 7? The same for Fig.8.

Figure 8b caption:  Six-pion prongs invariant -> Six-pion invariant

 question: do you use TPC or TOF pion hypothesis in the analysis? If yes then six-pion, if not then 6 prongs.

Summary:

We have presented -> It has been presented ; (there are couple of more "We"; avoid it; use passive voice)

modulation increases when increasing-> modulation increase when decreasing 

 excited rho in the ->  excited \rho in the

References:

 - check titles; there are mistakes like rho0 or n00n wrongly written

 - add commas between authors and titles, and journal names

 - for ref. 8 you should give an arxiv number

 - usually year is in round bracets, ie.: (2022) 
